The Planar Modular Partition Monoid

The primary contribution of this thesis is to introduce and examine the planar modular partition monoid for parameters $m, k \in \mathbb{Z}_{>0}$, which has simultaneously and independently generated interest from other researchers as outlined within. Our collective understanding of related monoids, in particular the Jones, Brauer and partition monoids, along with the algebras they generate, has heavily influenced the direction of research by a significant number of mathematicians and physicists. Examples include Schur-Weyl type dualities in representation theory along with Potts, ice-type and Andrew-Baxter-Forrester models from statistical mechanics, giving strong motivation for the planar modular partition monoid to be examined. The original results contained within this thesis relating to the planar modular partition monoid are: the establishment of generators; recurrence relations for the cardinality of the monoid; recurrence relations for the cardinality of Green's $\mathcal{R}$, $\mathcal{L}$ and $\mathcal{D}$ relations; and a conjecture on relations that appear to present the planar modular partition monoid when $m=2$. For diagram semigroups that are closed under vertical reflections, characterisations of Green's $\mathcal{R}$, $\mathcal{L}$ and $\mathcal{H}$ relations have previously been established using the upper and lower patterns of bipartitions. We give a characterisation of Green's $\mathcal{D}$ relation with a similar flavour for diagram semigroups that are closed under vertical reflections. $<paragraph\ missing\ due\ to\ arXiv\ character\ limit\ on\ abstracts\ -\ see\ thesis\ file>$ A further contribution of this thesis is a reasonably comprehensive exposition of the fundamentals of diagram semigroups, which have traditionally been approached from the representation theory side and have since blossomed into a thriving area of research in their own right.

==> chap_background/old/section_relations.tex <==
\section{Binary Relations}
        \begin{definition}
            A \textit{binary relation} on a set $X$ is a subset $\mathcal{R}$ of $X\times X$. We denote the set $\mathcal{P}(X\times{X})$ of binary relations on $X$ by $\mathcal{B}(X)$.
        \end{definition}
        
        \begin{definition}
            The \textit{composite} of two binary relations $\mathcal{L}$ and $\mathcal{R}$ on a set $X$ is the binary relation $\{(a, b) \in X\times{X}: \text{there exists } c \in X \text{ such that } (a, c) \in \mathcal{L} \text{ and } (c, b) \in \mathcal{R}\}$, which we denote by $\mathcal{R} \circ \mathcal{L}$.
        \end{definition}
        
        \begin{proposition}
        	The binary relations $\mathcal{B}(X)$ on a set $X$ are a monoid under composition with identity $\{(x,x): x \in X\}$.
        \end{proposition}
        
		Below we define some useful \textit{properties} of binary relations.            
         
        \begin{definition}
            A binary relation $\mathcal{R}$ on a set $X$ is:
            \begin{itemize}
                \item \textit{reflexive} if $(x, x) \in \mathcal{R}$ for all $x \in X$;
                \item \textit{symmetric} if $(x,y) \in \mathcal{R}$ implies $(y, x) \in \mathcal{R}$ for all $x, y \in X$;
                \item \textit{antisymmetric} if $(x,y) \in \mathcal{R}$ implies $(y, x)\ \cancel{\in}\ \mathcal{R}$ for all distinct $x, y \in X$;
                \item \textit{transitive} if $(x, y), (y, z) \in \mathcal{R}$ implies $(x, z) \in \mathcal{R}$ for all $x, y, z \in X$; and
                \item \textit{total} if for each $x , y \in X$, $(x, y) \in \mathcal{R}$ or $(y, x) \in \mathcal{R}$.
            \end{itemize}
        \end{definition}
        
        \begin{notation}
        	Let $P$ be a property of binary relations. We denote the set $\{\mathcal{R} \in \mathcal{B}(X): \mathcal{R} \text{ satisfies } P\}$ of binary relations satisfying $P$ as $\mathcal{B}_P(X)$.
        \end{notation}
        
		Often we will want to \textit{close} a binary relation so that it satisfies one of the above properties. Essentially this consists of further relating the smallest number of elements in a unique way such that the relevant property is satisfied, should this be possible. 
		
        \begin{definition}
        	Let $P$ be a property of binary relations and $\mathcal{R}$ be a binary relation. The $P$ \textit{closure} of $\mathcal{R}$, also called \textit{the $P$ binary relation generated by $\mathcal{R}$}, if it exists, is the smallest binary relation which contains $\mathcal{R}$ and satisfies $P$. We denote the $P$ closure of $\mathcal{R}$ as $<\mathcal{R}>^P$.
        \end{definition}
        
		As hinted in the definition, it does not always make sense to try and close every binary relation. For example a non-antisymmetric binary relation can not be antisymmetrically closed since it is not contained in any antisymmetric relations, and a non-total binary relation can not be totally closed since none of the many total binary relations which contain it are smallest. 
		
		If the $P$ closure exists for every binary relation then we say that $P$ is \textit{closable}. Below we give a characterisation of closability of properties. 
        
        \begin{proposition}
        	Let $X$ be a set. A binary relation property $P$ is closable if and only if the binary relations satisfying $P$ are closed under arbitrary intersections and $X\times\ X \in \mathcal{B}_P(X)$. Furthermore, the $P$ closure of a binary relation $\mathcal{R} \in \mathcal{B}(X)$ is equal to the intersection of the binary relations which contain $\mathcal{R}$ and satisfy $P$.
        	
        	\begin{proof}
        		First suppose the binary relations satisfying $P$ are closed under arbitrary intersections and $X\times\ X \in \mathcal{B}_P(X)$.
        		
        		For each $\mathcal{R} \in \mathcal{B}(X)$, $\{\mathcal{L} \in \mathcal{B}_P(X): \mathcal{R} \subseteq \mathcal{L}\}$ is non-empty, and for each $\mathcal{A} \in \{\mathcal{L} \in \mathcal{B}_P(X): \mathcal{R} \subseteq \mathcal{L}\}$, $\cap\{\mathcal{L} \in \mathcal{B}_P(X): \mathcal{R} \subseteq \mathcal{L}\} \subseteq \mathcal{A}$.
        		
        		Furthermore $\cap\{\mathcal{L} \in \mathcal{B}_P(X): \mathcal{R} \subseteq \mathcal{L}\} \in \mathcal{B}_P(X)$ since $\mathcal{B}_P(X)$ is closed under arbitrary intersections. Therefore the $P$ closure of $\mathcal{R}$ is equal to the intersection of the binary relations which contain $\mathcal{R}$ and satisfy $P$.
        		
        		Conversely, suppose $P$ is closable. Obviously $X\times{X} \in \mathcal{B}_P(X)$ since it is the only possible closure of itself. 
        		
        		Let $N$ be an index set and $\{\mathcal{R}_i \in \mathcal{B}_P(X): i \in N\}$ be a set of binary relations satisfying $P$. For each $j \in N$, $\cap_{i \in N} \mathcal{R}_i \subseteq \mathcal{R}_j$ and hence $<\cap_{i \in N} \mathcal{R}_i>^P\ \subseteq \mathcal{R}_j$.
        		
        		Therefore $<\cap_{i \in N} \mathcal{R}_i>^P\ \subseteq \cap_{i \in N} \mathcal{R}_i$, and hence $\mathcal{B}_P(X)$ is closed under arbitrary intersections.
        	\end{proof}
        \end{proposition}
        
        We note that each of the properties defined above except antisymmetry and totality are closable. Moreover, a property can be formed by a finite number of other properties $P_1$, ..., $P_n$ by simply requiring all properties be met. We shall refer to this property as the intersection of properties $P_1$, ..., $P_n$.  
        
        In such a case the set of binary relations satisfying the intersection of $P_1$, ..., $P_n$ is obviously equal to the intersection of the sets of binary relations satisfying each of the properties $P_1$, ..., $P_n$. Therefore we can unambiguously talk about the binary relations satisfying a finite number of properties without specifying whether we are talking about the set of binary relations satisfying all of the properties or the intersection of the sets of binary relations satisfying each property.     
        
        %\begin{proposition}
        	%Let $P_1, ..., P_n$ be properties of binary relations. The set of binary relations satisfying the intersection of properties $P_1, ..., P_n$ is equal to the intersection of the sets of binary relations satisfying each of the properties $P_1, ..., P_n$.
        	
        	%\begin{proof}
        		%$\mathcal{B}_{\cap^n_{i=1} P_i}(X) = \{\mathcal{R} \in \mathcal{B}(X): \mathcal{R} \text{ satisfies } P_1, ..., P_n\} = \cap^n_{i = 1}\{\mathcal{R} \in \mathcal{B}(X): \mathcal{R} \text{ satisfies } P_i\} = \cap^n_{i=1}\mathcal{B}_{P_i}(X)$
        	%\end{proof}
        %\end{proposition}

		\begin{proposition}
			If $P_1$, ..., $P_n$ is a finite number of closable binary relations then the intersection of $P_1$, ..., $P_n$ is also closable.
			\begin{proof}
				For each $1 \leq j \leq n$, since $X \times\ X \in \mathcal{B}_{P_j}(X)$, we have $X \times\ X \in \cap^n_{i=1} \mathcal{B}_{P_i}(X) = \mathcal{B}_{\cap^n_{i=1} P_i}(X)$.
				
				Let $N$ be an index set and $\{\mathcal{R}_i \in \mathcal{B}_{\cap^n_{i=1} P_i}(X): i \in N\} \subseteq \mathcal{B}_{P_1}(X), ..., \mathcal{B}_{P_n}(X)$ be a set of binary relations satisfying the intersection of the properties $P_1$, ..., $P_n$. 
				
				Since each property is closable, for each $1 \leq j \leq n$ we have $\cap_{i \in N} \mathcal{R}_i \in \mathcal{B}_{P_j}(X)$. Therefore $\cap_{i \in N} \mathcal{R}_i \in \mathcal{B}_{\cap^n_{j=1} P_j}(X)$.
			\end{proof}
		\end{proposition}
		
		Finally we show that there is no ambiguity in talking about the $P_1$, ..., $P_n$ closure of a finite number of binary relation properties.
        
		\begin{proposition}
			Let $P_1, ..., P_n$ be properties of binary relations and $\mathcal{R} \in \mathcal{B}(X)$. The closure of the intersection of $P_1$, ..., $P_n$ is equal to the iterated closure of each property individually. Furthermore, the order in which we close each property is irrelevant.
			\begin{proof}
				The first part follows from the set of binary relations satisfying a finite number of properties being equal to the intersection of the sets of binary relations satisfying each of the individual properties, and that the intersection of a finite number of closable binary relation properties is closable. 
				
				The second part follows from the closure of $P_1$, ..., $P_n$ remaining the same, regardless of the property ordering.
			\end{proof}
		\end{proposition}        
		
        
    \subsection{Order Relations}
        \begin{definition}
            A \textit{pre-order} on a set $X$ is a reflexive and transitive binary relation, in such a case we call $X$ a \textit{pre-ordered set}. A \textit{partial order} is an antisymmetric pre-order, in such a case we call $X$ a \textit{partially ordered set}. 
        \end{definition}
      	
      	Since partial orders are antisymmetric, there cannot exist distinct elements with the same order, so we need not bother considering their existence. 
      	
      	\begin{definition}
        	Let $X$ be a partially ordered set and $S \subseteq X$. An element $x \in S$ is: \textit{greatest} if it is greater than or equal to every other element in $S$; \textit{least} if it is smaller than or equal to every other element in $S$; \textit{maximal} if there does not exist another element in $S$ which is smaller than $x$; and \textit{minimal} if there does not exist an element in $S$ which is larger than $x$.
        \end{definition}
      	
      	\begin{definition}
      		A \textit{total order} is a total partial order. A \textit{chain} is a totally ordered subset of a partially ordered set. 
      	\end{definition}
        
        
    \subsection{Equivalence Relations}
        
        \begin{definition}
            An \textit{equivalence relation} is a reflexive, symmetric and transitive binary relation.
        \end{definition}
        
        \begin{notation}
       		We denote the equivalence relation generated by a binary relation $\mathcal{R}$ as $<\mathcal{R}>$.
       	\end{notation}
        
        \begin{definition}
            Let $\sim$ be an equivalence relation on a set $X$. The \textit{equivalence class} of $x \in X$ is the set $\{y \in X: y \sim x\}$ which we denote by $[x]$. The set of equivalence classes $\{[x]: x \in X\}$ is a partition of $X$, which is called the \textit{quotient set} and is denoted by $X/{\sim}$.
        \end{definition}
        
		\begin{proposition}
			If $\mathcal{R}$ is a binary relation on a set $X$ then $\{(x, x'): \text{ there} \newline \text{exists } a_1, ..., a_n \in X \text{ such that } x = a_1, x' = a_n, \text{ and } (a_1, a_2), ..., (a_{n-1}, a_n) \in \mathcal{R}\}$ is the equivalence relation generated by $\mathcal{R}$.
		\end{proposition}        
        
		\begin{definition}
			Let $\mathcal{R}_1, ..., \mathcal{R}_n$ be binary relations on a set $X$. The \textit{equivalence relation generated by } $\mathcal{R}_1, ..., \mathcal{R}_n$ is $<\cup^n_{i=1}\mathcal{R}_i>$ which we denote by $<\mathcal{R}_1, ..., \mathcal{R}_n>$.
		\end{definition}
        
        Often we will want to consider the equivalence relations on an algebraic object which have a well-defined operation on its equivalence classes. These are captured with congruence relations but their exact definition varies depending on the relevant algebraic object. These will be defined as necessary later on, however they can be classified generally as follows: the product of two equivalence classes should be uniquely inferable from any representative elements of the classes. 
        
       	\begin{notation}
       		We denote the congruence relation generated by a binary relation $\mathcal{R}$ as $<\mathcal{R}>^{\cong}$.
       	\end{notation}
	

==> chap_background/old/section_semigroups.tex <==
\section{Semigroups}
	    \begin{definition}
	      A \textit{semigroup} consists of a set together with an associative binary relation. Unless otherwise specified we let $S$ be a semigroup.
	    \end{definition}
	    
	    \begin{notation}
	      Let $X$ be a set. For $a \in X$ and $B \subseteq X$ we denote the set $\{ab: b \in B\}$ as $aB$ and similarly the set $\{ba: b \in B\}$ as $Ba$. For subsets $A, B \subseteq X$ we denote the set $\{ab: a \in A \text{ and } b \in B\}$ as $AB$. 
	    \end{notation}
		    
	    \begin{definition}
	    	A subset $T \subseteq S$ is a \textit{subsemigroup} of $S$ if $TT \subseteq T$, denoted by $T \leq S$.
	    \end{definition}
		    
	    \begin{definition}
	    	A semigroup is regular if for each $x \in S$ there exists $y \in S$ such that $xyx = x$ and $yxy = y$.
	    \end{definition}
	
		    
	\subsection{Regular $^*$-Semigroups}
	    \begin{definition}
	        An \textit{involution} is a unary operation $^*:S\rightarrow{S}$ which is:
	        \begin{enumerate}
	            \item its own inverse ($(x^*)^* = x$ for all $x \in S$); and
	            \item an anti-automorphism ($(xy)^* = y^*x^*$ for all $x, y \in S$).
	        \end{enumerate}
	        
	        A \textit{semigroup with involution}, also called a \textit{$^*$-semigroup}, is a semigroup with an involution $^*$. Furthermore if $xx^*x = x$ for all $x \in S$ then it is called a \textit{regular $^*$-semigroup}.
	    \end{definition}
	    
	    %question: can there exist a *-semigroup which is regular but isn't a regular *-semigroup?
	    
	    \begin{definition}
	        A \textit{projection} for a regular $^*$-semigroup $S$ is an element $p \in S$ satisfying $p^2 = p = p^*$.
	    \end{definition}
	    
	    \begin{proposition}
	        The projections (and more generally idempotents) of a regular $^*$-semigroup are partially ordered by $p \leq q$ if and only if $pq = p = qp$.
	        \begin{proof}
	        	Clearly $\leq$ is reflexive and antisymmetric leaving transitivity. Let $p, q, r \in S$ such that $p \leq q \leq r$. Then $pr = (pq)r = p(qr) = pq = p = qp = rqp = rp$.
	        \end{proof}
	    \end{proposition}
	    
	    \begin{proposition}
	        In a regular $^*$-semigroup $S$:
	        \begin{enumerate}
	            \item for each $x \in X$, $xx^*$ is a projection; 
	            \item every projection is of the above form;
	            \item idempotents are closed under involution;
	            \item every idempotent is the product of two projections; and
	            \item for each $x, y \in S$, $x \in Sy$ if and only if $x^*x \leq y^*y$.
	        \end{enumerate}
	        
	        \begin{proof}
	        	\begin{enumerate}
	        		\item For each $x \in X$, $(xx^*)(xx^*) = (xx^*x)x^* = xx^* = (x^*)^*x^* = (xx^*)^*$.
	        		\item For each projection $p \in S$ we trivially have $p = p^2 = pp^*$.
	        		\item For each idempotent $e \in S$, $e^*e^* = (ee)^* = e^*$.
	        		\item For each idempotent $e \in S$, $(e^*e)^*(e^*e) = ee^*e^*e = ee^*e = e$.
	        		\item Let $x, y \in S$. suppose there exists $s \in S$ such that $sy = x$. Then $(x^*x)(y^*y) = y^*s^*syy^*y = y^*s^*sy = x^*x = y^*s^*sy = y^*yy^*s^*sy = (y^*y)(x^*x)$. 
	        		
	        		Conversely, suppose $x^*x \leq y^*y$, then $xy^*y = xx^*xy^*y = xx^*x = x$.
	        	\end{enumerate}
	        \end{proof}
	    \end{proposition}
	    
	\subsection{Ideals}
	    \begin{definition}
	        A subset $I \subseteq S$ is:
	        \begin{itemize}
	            \item a \textit{left ideal} if $SI \subseteq I$;
	            \item a \textit{right ideal} if $IS \subseteq I$; and
	            \item an \textit{ideal} if it is a left and right ideal.
	        \end{itemize}
	    \end{definition}
	    
	    %Since $S \times S$ is always a left, right and two-sided ideal, and ideals are closed under arbitrary intersections, it follows that 
	    
	    \begin{proposition}
	        For each $a \in S$:
	        \begin{enumerate}
	            \item $Sa \cup \{a\}$ is a left ideal;
	            \item $aS \cup \{a\}$ is a right ideal; and
	            \item $SaS \cup \{a\}$ is an ideal.
	        \end{enumerate}
		        
	        \begin{proof}
	        	For each $a \in S$ we have:
	            \begin{enumerate}
	            	\item $(Sa \cup \{a\})(Sa \cup \{a\}) = (Sa)(Sa) \cup (Sa)a \cup a(Sa) \cup aa \subseteq Sa \cup \{a\}$ and $S(Sa \cup \{a\}) = (SS)a \cup Sa \subseteq Sa \cup \{a\}$;
	            	\item $(aS \cup \{a\})(aS \cup \{a\}) = (aS)(aS) \cup (aS)a \cup a(aS) \cup aa \subseteq aS \cup \{a\}$ and $(aS \cup \{a\})S = a(SS) \cup aS \subseteq Sa \cup \{a\}$; and
	            	\item $(SaS \cup \{a\})(SaS \cup \{a\}) = (SaS)(SaS) \cup (SaS)a \cup a(SaS) \cup aa \subseteq SaS \cup \{a\}$ and $S(SaS \cup \{a\})S = (SS)a(SS) \cup SaS \subseteq SaS \cup \{a\}$.
	            \end{enumerate}
	        \end{proof}
	    \end{proposition}
	    
	    \begin{definition}
	        Let $a \in S$. $Sa \cup \{a\}$ is the \textit{principal left ideal generated by $a$} , $aS \cup \{a\}$ is the \textit{principal right ideal generated by $a$} and $SaS \cup \{a\}$ is the \textit{principal ideal generated by $a$}.
	    \end{definition}
	    
	    %\begin{proposition}
	    	%If $I, J \subseteq S$ are (left/right/two-sided) ideals then $I \cup J$ is a (left/right/two-sided) ideal.
	    %\end{proposition}
	    
	    %\begin{proposition}
	    	%If $I \subseteq S$ is an ideal then there exists principal ideals $I_1, ..., I_n$ such that $I = \cup^n_{i=1} I_i$.
	    %\end{proposition}
		
	\subsection{Green's Relations}
	    \begin{definition}
	        For each $a, b \in S$, $(a, b) \in \leq_{\mathcal{L}}$ if and only if $Sa \cup \{a\} \subseteq Sb \cup \{b\}$ and $(a, b) \in \leq_{\mathcal{R}}$ if and only if $aS \cup \{a\} \subseteq bS \cup \{b\}$.
	    \end{definition}
		    
	    \begin{proposition}
	        $\leq_{\mathcal{L}}$ and $\leq_{\mathcal{R}}$ are pre-orders on $S$.
		        
	        \begin{proof}
	            Reflexivity is obvious and transitivity follows from $\subseteq$ being transitive on sets.
	        \end{proof}
	    \end{proposition}
		
	    \begin{definition}
	        Green's relations on a semigroup $S$ are defined by:
	        \begin{itemize}
	            \item $\mathcal{L} = \leq_{\mathcal{L}} \cap \leq_{\mathcal{L}}^{-1} = \{(a, b) \in S \times S: Sa \cup \{a\} = Sb \cup \{b\}\}$;
	            \item $\mathcal{R} = \leq_{\mathcal{R}} \cap \leq_{\mathcal{R}}^{-1} = \{(a, b) \in S \times S: aS \cup \{a\} = bS \cup \{b\}\}$;
	            \item $\mathcal{H} = \mathcal{L} \cap \mathcal{R}$;
	            \item $\mathcal{D} = \{(a, b) \in S\times S: \text{there exists } c \in S \text{ such that } a \mathcal{L} c \text{ and } c \mathcal{R} b\}$; and
	            \item $\mathcal{J} = \{(a, b) \in S\times S: SaS \cup \{a\} = SbS \cup \{b\}\}$.
	        \end{itemize}
	    \end{definition}
		    
		  Green's $\mathcal{L}$, $\mathcal{R}$ and $\mathcal{H}$ relations on regular submonoids of a monoid are just their respective restrictions of those on $\mathcal{P}_n$, see \cite{Hall} and \cite{Howie}.

				\begin{theorem} \label{HowieThm}
					If $T \leq S$ is regular then Green's $\mathcal{L}$, $\mathcal{R}$ and $\mathcal{H}$ relations are just their respective restrictions on $S$. Ie. $\mathcal{L}^T$ = $\mathcal{L}^S \cap T^2$.
				\end{theorem}		    
		    
        %\begin{proposition}
            %$\mathcal{J} \subseteq \mathcal{D} \subseteq \mathcal{L}, \mathcal{R} \subseteq \mathcal{H}$.
        %\end{proposition}
	        
        %\begin{proposition}
            %$\mathcal{H} = \mathcal{L} \circ \mathcal{R} = \mathcal{R} \circ \mathcal{L}\ ( = \mathcal{L} \vee \mathcal{R})$.
        %\end{proposition}
	        
        %\begin{proposition}
            %$S/{\mathcal{R}}$ is partially ordered by $\leq_{\mathcal{R}}$.
        %\end{proposition}
	
	    %\begin{proposition}
	        %If $T \leq S$ then $\mathcal{L}_T \subseteq \mathcal{L}_S$
	    %\end{proposition}
		    
	    %\begin{proposition}
	        %If $T \leq S$ is regular then $a \mathcal{L}_S b$ implies $a \mathcal{L}_T b$ for all $a, b \in T$.
	    %\end{proposition}
	    
	\subsection{Semigroup Congruences \& Factor Semigroups}
		Often we will want to consider the equivalence classes of an equivalence relation as themselves being a semigroup. Below we outline a characterisation of when this is possible.
		
		\begin{definition}
			A \textit{semigroup congruence} on a semigroup $S$ is an equivalence relation $\cong$ on $S$ such that for all $a, b, c, d \in S$, if $(a, b) \in \cong$ and $(c, d) \in \cong$ then $(ac, bd) \in \cong$, or equivalently if $b \in [a]$ and $d \in [c]$ then $bd \in [ac]$. The equivalence classes of a semigroup congruence are called \textit{congruence classes}.
		\end{definition}		
		
		\begin{proposition}
			Let $\mathcal{R}$ be a binary relation on a semigroup $S$. The congruent closure of $\mathcal{R}$ exists, which we denote by $<\mathcal{R}>^{\cong}$. 
			
			\begin{proof}
				$S \times\ S$ is obviously a congruence relation. Let $N$ be an index set and $\{\cong_i \in \mathcal{B}_{\cong}(X): i \in N\}$ be a set of congruence relations. Let $a, b, c, d \in X$ such that $(a, c), (b, d) \in \cap_{i \in N} \cong_i$. Then for each $i \in N$ we have $(ac, bd) \in \cong_i$ and hence the result follows.
			\end{proof}
		\end{proposition}
		
		
		
		We show that for an equivalence relation which is not a semigroup congruence there does not exist a representative-independent way to \textit{multiply} equivalence classes based on representative elements.
		
		\begin{proposition}
		 	If $\sim$ is an equivalence relation on a semigroup $S$ which is not a semigroup congruence then there exists $a, c \in S$ such that $[a][c] \nsubseteq [s]$ for all $s \in S$. 
		 	
		 	\begin{proof}
		 		Since $\sim$ is not a semigroup congruence there exists $a, b, c, d \in S$ such that $b \in [a]$, $d \in [c]$ and $bd\ \cancel{\in}\ [ac]$.  Therefore we have $ac, bd \in [a][c]$, $ac \in [ac]$ and $bd\ \cancel{\in}\ [ac]$, so $[a][c]$ is not a subset of any of the equivalence classes.
		 	\end{proof}
		\end{proposition}
		
		Next we show that for a congruence relation, the product of two congruence classes is contained in the congruence class of the product of an arbitrary representative element from each class. 		
		
		\begin{proposition}
			If $\cong$ is a semigroup congruence then $[s][s'] \subseteq [ss']$ for all $s, s' \in S$.
			
			\begin{proof}
				Let $t \in [s]$ and $t' \in [s']$, since $\cong$ is a semigroup congruence we have $tt' \in [ss']$ as required.
			\end{proof}
		\end{proposition}
		
		Restricting the set product to congruence classes is not an operation on congruence classes, to obtain this we must make the following definition. 
		
		\begin{definition}
			Let $\cong$ be a semigroup congruence on a semigroup $S$. We define an operation $*$ on the congruence classes by $[s]*[s'] = [ss']$ for all $s, s' \in S$. 
		\end{definition}		
		
		\begin{proposition}
			Let $\cong$ be a semigroup congruence on a semigroup $S$. The congruence classes form a semigroup under the operation $*$ as defined above.
			
			\begin{proof}
				The operation is closed since for each $s, s' \in S$ we have $[s]*[s'] = [ss']$, which just leaves associativity. 
				
				For each $s, s', s'' \in S$ we have $([s]*[s'])*[s''] = [ss']*[s''] = [ss's''] = [s]*[s's''] = [s]*([s']*[s''])$.
			\end{proof}
		\end{proposition}
		
		
		  
    \subsection{Presentations}
	    \begin{definition}
	        The \textit{free semigroup} on a set $S$, which we denote by $S^*$, is the semigroup $\cup_{n \in \mathbb{Z}^+} S^n$ of finite strings of elements of $S$ together with string concatenation.
	    \end{definition}
	
	    \begin{definition}
	        A \textit{presentation} of a semigroup $S$ consists of:
	        \begin{enumerate}
	            \item a set $\Sigma \subseteq S$ of generators; and 
	            \item a set $\{\mathcal{R}_1, ..., \mathcal{R}_n\}$ of binary relations on the free semigroup $\Sigma^*$ on $\Sigma$;
	        \end{enumerate}
	        such that $S = \Sigma^*/{\mathcal{R}}$ where $\mathcal{R} = <\mathcal{R}_1, ..., \mathcal{R}_n>^{\cong}$.
	    \end{definition}
		    

==> chap_background/tikz/old/F5generators.tex <==
\begin{figure}[!ht]
  \caption{The three generators of $\mathcal{J}_4$.}
  \label{J4Generators}
	\vspace{10pt}
	\centering
  \scalebox{1}
  {
    \begin{pspicture}(0,-0.88)(2.54,0.88)
    \psdots[dotsize=0.12](0.06,0.8)
    \psdots[dotsize=0.12](1.26,-0.8)
    \psdots[dotsize=0.12](2.46,0.8)
    \psdots[dotsize=0.12](2.46,-0.8)
    \psdots[dotsize=0.12](0.06,-0.8)
    \psdots[dotsize=0.12](0.66,-0.8)
    \psdots[dotsize=0.12](1.86,-0.8)
    \psdots[dotsize=0.12](1.86,0.8)
    \psdots[dotsize=0.12](0.66,0.8)
    \psdots[dotsize=0.12](1.26,0.8)
    \psline[linewidth=0.04cm](1.26,0.8)(1.26,0.2)
    \psline[linewidth=0.04cm](1.26,-0.8)(1.26,-0.2)
    \psline[linewidth=0.04cm](1.26,-0.2)(2.46,-0.2)
    \psline[linewidth=0.04cm](2.46,-0.2)(2.46,-0.8)
    \psline[linewidth=0.04cm](1.86,-0.8)(1.86,-0.2)
    \psline[linewidth=0.04cm](1.86,0.8)(1.86,0.2)
    \psline[linewidth=0.04cm](2.46,0.8)(2.46,0.2)
    \psline[linewidth=0.04cm](1.26,0.2)(2.46,0.2)
    \psline[linewidth=0.04cm](0.06,0.8)(0.06,-0.8)
    \psline[linewidth=0.04cm](0.66,0.8)(0.66,-0.8)
    \end{pspicture} ,
    \begin{pspicture}(0,-0.88)(2.54,0.88)
    \psdots[dotsize=0.12](0.06,0.8)
    \psdots[dotsize=0.12](1.26,-0.8)
    \psdots[dotsize=0.12](2.46,0.8)
    \psdots[dotsize=0.12](2.46,-0.8)
    \psdots[dotsize=0.12](0.06,-0.8)
    \psdots[dotsize=0.12](0.66,-0.8)
    \psdots[dotsize=0.12](1.86,-0.8)
    \psdots[dotsize=0.12](1.86,0.8)
    \psdots[dotsize=0.12](0.66,0.8)
    \psdots[dotsize=0.12](1.26,0.8)
    \psline[linewidth=0.04cm](1.26,0.8)(1.26,0.2)
    \psline[linewidth=0.04cm](1.26,-0.8)(1.26,-0.2)
    \psline[linewidth=0.04cm](1.26,-0.2)(2.46,-0.2)
    \psline[linewidth=0.04cm](2.46,-0.2)(2.46,-0.8)
    \psline[linewidth=0.04cm](1.86,-0.8)(1.86,-0.2)
    \psline[linewidth=0.04cm](1.86,0.8)(1.86,0.2)
    \psline[linewidth=0.04cm](2.46,0.8)(2.46,0.2)
    \psline[linewidth=0.04cm](1.26,0.2)(2.46,0.2)
    \psline[linewidth=0.04cm](0.06,0.8)(0.06,-0.8)
    \psline[linewidth=0.04cm](0.66,0.8)(0.66,-0.8)
    \end{pspicture} ,
    \begin{pspicture}(0,-0.88)(2.54,0.88)
    \psdots[dotsize=0.12](0.06,0.8)
    \psdots[dotsize=0.12](1.26,-0.8)
    \psdots[dotsize=0.12](2.46,0.8)
    \psdots[dotsize=0.12](2.46,-0.8)
    \psdots[dotsize=0.12](0.06,-0.8)
    \psdots[dotsize=0.12](0.66,-0.8)
    \psdots[dotsize=0.12](1.86,-0.8)
    \psdots[dotsize=0.12](1.86,0.8)
    \psdots[dotsize=0.12](0.66,0.8)
    \psdots[dotsize=0.12](1.26,0.8)
    \psline[linewidth=0.04cm](1.26,0.8)(1.26,0.2)
    \psline[linewidth=0.04cm](1.26,-0.8)(1.26,-0.2)
    \psline[linewidth=0.04cm](1.26,-0.2)(2.46,-0.2)
    \psline[linewidth=0.04cm](2.46,-0.2)(2.46,-0.8)
    \psline[linewidth=0.04cm](1.86,-0.8)(1.86,-0.2)
    \psline[linewidth=0.04cm](1.86,0.8)(1.86,0.2)
    \psline[linewidth=0.04cm](2.46,0.8)(2.46,0.2)
    \psline[linewidth=0.04cm](1.26,0.2)(2.46,0.2)
    \psline[linewidth=0.04cm](0.06,0.8)(0.06,-0.8)
    \psline[linewidth=0.04cm](0.66,0.8)(0.66,-0.8)
    \end{pspicture}.
  }
\end{figure}

==> chap_background/tikz/old/PatternExample.tex <==
\begin{tikzpicture} [scale = 0.6]
  \draw(4, 2.05) node [above] {{$\alpha$}};

  %block #1
  %vertices and labels
  \fill(1,2)circle(.125);
  \fill(1,0)circle(.125);
  \fill(2,0)circle(.125);
  \fill(3,0)circle(.125);

  %lines
  \draw(1,0.125) .. controls (1,0.571429) and (2,0.571429) .. (2,0.125);
  \draw(2,0.125) .. controls (2,0.571429) and (3,0.571429) .. (3,0.125);
  \draw(1,2)--(1,0);

  %block #2
  %vertices and labels
  \fill(2,2)circle(.125);
  \fill(6,2)circle(.125);
  \fill(7,2)circle(.125);
  \fill(4,0)circle(.125);

  %lines
  \draw(2,1.875) .. controls (2,1.21429) and (6,1.21429) .. (6,1.875);
  \draw(6,1.875) .. controls (6,1.42857) and (7,1.42857) .. (7,1.875);
  \draw(2,2)--(4,0);

  %block #3
  %vertices and labels
  \fill(3,2)circle(.125);
  \fill(4,2)circle(.125);
  \fill(5,2)circle(.125);

  %lines
  \draw(3,1.875) .. controls (3,1.42857) and (4,1.42857) .. (4,1.875);
  \draw(4,1.875) .. controls (4,1.42857) and (5,1.42857) .. (5,1.875);

  %block #4
  %vertices and labels
  \fill(5,0)circle(.125);
  \fill(6,0)circle(.125);
  \fill(7,0)circle(.125);

  %lines
  \draw(5,0.125) .. controls (5,0.571429) and (6,0.571429) .. (6,0.125);
  \draw(6,0.125) .. controls (6,0.571429) and (7,0.571429) .. (7,0.125);

\draw(8,2.6)--(8,-0.6);

%upper pattern
  \draw(12, 2.05) node [above] {{$U(\alpha)$}};
  \fill(9,2)circle(.125);
  \fill(10,2)circle(.125);
  \draw(11,2)circle(.115);
  \draw(12,2)circle(.115);
  \draw(13,2)circle(.115);
  \fill(14,2)circle(.125);
  \fill(15,2)circle(.125);

  \draw (10,1.875) .. controls (10,1.21429) and (14,1.21429) .. (14,1.875);
  \draw (14,1.875) .. controls (14,1.42857) and (15,1.42857) .. (15,1.875);
  \draw (11,1.875) .. controls (11,1.42857) and (12,1.42857) .. (12,1.875);
  \draw (12,1.875) .. controls (12,1.42857) and (13,1.42857) .. (13,1.875);
  
%lower pattern
  \draw(12, -0.05) node [below] {{$L(\alpha)$}};
  \fill(9,0)circle(.125);
  \fill(10,0)circle(.125);
  \fill(11,0)circle(.125);
  \fill(12,0)circle(.125);
  \draw(13,0)circle(.115);
  \draw(14,0)circle(.115);
  \draw(15,0)circle(.115);

  \draw (9,0.125) .. controls (9,0.57143) and (10,0.57143) .. (10,0.125);
  \draw (10,0.125) .. controls (10,0.57143) and (11,0.57143) .. (11,0.125);
  \draw (13,0.125) .. controls (13,0.57143) and (14,0.57143) .. (14,0.125);
  \draw (14,0.125) .. controls (14,0.57143) and (15,0.57143) .. (15,0.125);
\end{tikzpicture}

==> chap_background/tikz/old/ProductExample.tex <==
\begin{tikzpicture}[scale = 0.6]
  %block #1
  %vertices and labels
  %\fill(colNo[1-5], rowNo[2/0])circle(0.125)
  \fill(1,4)circle(.125);
  \fill(5,4)circle(.125);
  \fill(4,2)circle(.125);
  \fill(5,2)circle(.125);

  %lines
  \draw(1,3.875) .. controls (1,3.1) and (5,3.1) .. (5,3.875);
  \draw(4,2.125) .. controls (4,2.6) and (5,2.6) .. (5,2.125);
  \draw(5,4)--(5,2);

  %block #2
  %vertices and labels
  \fill(2,4)circle(.125);
  \fill(3,4)circle(.125);
  \fill(4,4)circle(.125);

  %lines
  \draw(2,3.875) .. controls (2,3.4) and (3,3.4) .. (3,3.875);
  \draw(3,3.875) .. controls (3,3.4) and (4,3.4) .. (4,3.875);

  %block #3
  %vertices and labels
  \fill(1,2)circle(.125);

  %lines

  %block #4
  %vertices and labels
  \fill(2,2)circle(.125);
  \fill(3,2)circle(.125);

  %lines
  \draw(2,2.125) .. controls (2,2.6) and (3,2.6) .. (3,2.125);
%%%

  %block #1
  %vertices and labels
  \fill(1,2)circle(.125);
  \fill(4,2)circle(.125);
  \fill(5,2)circle(.125);
  \fill(1,0)circle(.125);
  \fill(2,0)circle(.125);
  \fill(3,0)circle(.125);

  %lines
  \draw(1,1.875) .. controls (1,1.2) and (4,1.2) .. (4,1.875);
  \draw(4,1.875) .. controls (4,1.4) and (5,1.4) .. (5,1.875);
  \draw(1,0.125) .. controls (1,0.6) and (2,0.6) .. (2,0.125);
  \draw(2,0.125) .. controls (2,0.6) and (3,0.6) .. (3,0.125);
  \draw(1,2)--(1,0);

  %block #2
  %vertices and labels
  \fill(2,2)circle(.125);
  \fill(3,2)circle(.125);

  %lines
  \draw(2,1.875) .. controls (2,1.4) and (3,1.4) .. (3,1.875);

  %block #3
  %vertices and labels
  \fill(4,0)circle(.125);
  \fill(5,0)circle(.125);

  %lines
  \draw(4,0.125) .. controls (4,0.6) and (5,0.6) .. (5,0.125);
%%%
  \draw(6, 2) node {{$=$}};

  %block #1
  %vertices and labels
  \fill(7,3)circle(.125);
  \fill(11,3)circle(.125);
  \fill(7,1)circle(.125);
  \fill(8,1)circle(.125);
  \fill(9,1)circle(.125);

  %lines
  \draw(7,2.875) .. controls (7,2.1) and (11,2.1) .. (11,2.875);
  \draw(7,1.125) .. controls (7,1.6) and (8,1.6) .. (8,1.125);
  \draw(8,1.125) .. controls (8,1.6) and (9,1.6) .. (9,1.125);
  \draw(7,3)--(7,1);

  %block #2
  %vertices and labels
  \fill(8,3)circle(.125);
  \fill(9,3)circle(.125);
  \fill(10,3)circle(.125);

  %lines
  \draw(8,2.875) .. controls (8,2.4) and (9,2.4) .. (9,2.875);
  \draw(9,2.875) .. controls (9,2.4) and (10,2.4) .. (10,2.875);

  %block #3
  %vertices and labels
  \fill(10,1)circle(.125);
  \fill(11,1)circle(.125);

  %lines
  \draw(10,1.125) .. controls (10,1.6) and (11,1.6) .. (11,1.125);
\end{tikzpicture}


==> chap_cardinalities/old/chap_cardinalities.tex <==
\chapter{Cardinalities}
    \section{Known Cardinalities}
		\begin{table}[!ht]
            \caption{Cardinalities ...}
            \tiny
            \centering
            \begin{tabular}{|c|cccc|}
            \hline
            OEI & A000110* 		& A000108* 				& A000142 		&  \\
            \hline
            $k$ & $|\pttnmon{k}|$ 	& $|\ppttnmon{k}|$ 	& $|\symgrp{k}|$ 	& $|\transmon{k}|$ \\
            \hline
            1	& 2            & 2         & 1      & \\
            2	& 15           & 14        & 2      & \\
            3	& 203          & 132       & 6      & \\
            4	& 4140         & 1430      & 24     & \\
            5	& 115975       & 16796     & 120    & \\
            6	& 4213597      & 208012    & 720    & \\
            7	& 190899322    & 2674440   & 5040   & \\
            8	& 10480142147  & 35357670  & 40320  & \\
            9	& 682076806159 & 477638700 & 362880 & \\
            \hline
            \end{tabular}
        \end{table}

  	\section{Jones monoids $|\jonesmon{k}|$ and Brauer monoid $|\brauermon{k}|$}
  		Planning to have a discussion here about how we already know the cardinalities (with references) and that this is to give the reader a simpler example of how we will count the triapsis and Fauser monoids. 
  	
  		Let $J(k, d)$ be the number of $\jonesmon{k}$-admissible patterns with $d$ diapses. Similarly, let $B(k, d)$ be the number of $\brauermon{k}$-admissible patterns with $d$ diapses. 
  		
  		\begin{proposition} 
  			The numbers $J(k, d)$ satisfy the recurrence:
  			\[ J(k, d) =
  								\begin{cases}
   								1 													& \text{ if } d = 0 \\
   								J(k-1, d) + J(k-1, d-1)    & \text{ if } 1 \leq d \leq \lfloor \frac{k}{2} \rfloor \\
   								0													& \text{ otherwise } 
  								\end{cases} \]
  			and the numbers $B(k, d)$ satisfy the recurrence:
  			\[ B(k, d) =
  								\begin{cases}
   								1 																			 & \text{ if } d = 0 \\
   								B(k-1, d) + (k-1)B(k-2, d-1)    & \text{ if } 1 \leq d \leq \lfloor \frac{k}{2} \rfloor \\
   								0																				 & \text{ otherwise } 
  								\end{cases} \]
  								
  			\begin{proof}
  				When $d = 0$ every vertex is a singleton, hence both $J(k, 0)$ and $B(k, 0)$ are equal to $1$. When $1 \leq d \leq \lfloor \frac{k}{2} \rfloor$ , if no diapses connect to the right-most vertex then there are $J(k-1, d)$ and $B(k-1, d)$ such patterns for $\jonesmon{k}$ and $\brauermon{k}$ respectively. If there is a diapsis connected to the right-most vertex: for the $\jonesmon{k}$-admissible patterns with $d$ diapses, there are $J(k-1, d-1)$ ways to add $d-1$ diapses to the first $k-1$ vertices, to which we can connect the two right-most vertices yet to have a diapsis attached; and for the $\brauermon{k}$-admissible patterns with $d$ diapses, for each of the $k-1$ vertices the right-most vertex can connect to, there are $B(k-2, d-1)$ possible ways to add $d-1$ diapses to the remaining $k-2$ vertices. 
			\end{proof}
		\end{proposition}
		
		\begin{theorem}
  			The cardinalities of $\jonesmon{k}$ and $\brauermon{k}$ are given by:
  			\[ |\jonesmon{k}| = \Sigma_{d=0}^{\lfloor k/2 \rfloor} J(k, d)^2 \text{, and } |\brauermon{k}| = \Sigma_{d=0}^{\lfloor k/2 \rfloor}(k-2d)!B(k, d)^2 \]
  			\begin{proof}
  				For two $\jonesmon{k}$-admissible patterns to be compatible they need to contain the same number of diapses, and given two $\jonesmon{k}$-admissible patterns $p$ and $q$ there is a distinct diagram $\alpha \in \jonesmon{k}$ such that $\uppat{\alpha} = p$ and $\lowpat{\alpha} = q$. The only difference with $\brauermon{k}$ is that given two $\brauermon{k}$-admissible patterns $p$ and $q$, both with $d$ diapses, there are $(k-2d)!$ diagrams $\alpha \in \brauermon{k}$ such that $\uppat{\alpha} = p$ and $\lowpat{\alpha} = q$.
  			\end{proof}
  		\end{theorem}
  		
		\begin{table}[!ht] \label{tab:Jadmispatternswithddiapes}
  			\caption{Example values for $J(k, d)$ and $|\jonesmon{k}|$.}
  			\centering
  			\tiny
		    \begin{tabular}{|c|rrrrrrrr|c|}
				\hline
				\diagbox{k}{d} & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & $|\jonesmon{k}|$ \\
				\hline
				0 & 1 &   &   &   &   &   &   &   & 0 \\
				1 & 1 &   &   &   &   &   &   &   & 1 \\
				2 & 1 & 1 &   &   &   &   &   &   & 2 \\
				3 & 1 & 2 &   &   &   &   &   &   & 5 \\
				4 & 1 & 3 & 2 &   &   &   &   &   & 14 \\
				5 & 1 & 4 & 5 &   &   &   &   &   & 42 \\
				6 & 1 & 5 & 9 & 5 &   &   &   &   & 132 \\
				7 & 1 & 6 & 14 & 14 &   &   &   &   & 429 \\
				8 & 1 & 7 & 20 & 28 & 14 &   &   &   & 1430 \\
				9 & 1 & 8 & 27 & 48 & 42 &   &   &   & 4862 \\
				10 & 1 & 9 & 35 & 75 & 90 & 42 &   &   & 16796 \\
				11 & 1 & 10 & 44 & 110 & 165 & 132 &   &   & 58786 \\
				12 & 1 & 11 & 54 & 154 & 275 & 297 & 132 &   & 208012 \\
				13 & 1 & 12 & 65 & 208 & 429 & 572 & 429 &   & 742900 \\
				14 & 1 & 13 & 77 & 273 & 637 & 1001 & 1001 & 429 & 2674440 \\
				15 & 1 & 14 & 90 & 350 & 910 & 1638 & 2002 & 1430 & 9694845 \\
				\hline
			\end{tabular}
		\end{table}

		\begin{table}[!ht] \label{tab:Badmispatternswithddiapes}
  			\caption{Example values for $B(k, d)$ and $|\brauermon{k}|$.}
  			\centering
  			\tiny
			\begin{tabular}{|c|rrrrrrrr|c|}
				\hline
				\diagbox{k}{d} & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & $|\brauermon{k}|$ \\
				\hline
				0 & 1 &   &   &   &   &   &   &   & 0 \\
				1 & 1 &   &   &   &   &   &   &   & 1 \\
				2 & 1 & 1 &   &   &   &   &   &   & 3 \\
				3 & 1 & 3 &   &   &   &   &   &   & 15 \\
				4 & 1 & 6 & 3 &   &   &   &   &   & 105 \\
				5 & 1 & 10 & 15 &   &   &   &   &   & 945 \\
				6 & 1 & 15 & 45 & 15 &   &   &   &   & 10395 \\
				7 & 1 & 21 & 105 & 105 &   &   &   &   & 135135 \\
				8 & 1 & 28 & 210 & 420 & 105 &   &   &   & 2027025 \\
				9 & 1 & 36 & 378 & 1260 & 945 &   &   &   & 34459425 \\
				10 & 1 & 45 & 630 & 3150 & 4725 & 945 &   &   & 654729075 \\
				11 & 1 & 55 & 990 & 6930 & 17325 & 10395 &   &   & 13749310575 \\
				12 & 1 & 66 & 1485 & 13860 & 51975 & 62370 & 10395 &   & 316234143225 \\
				13 & 1 & 78 & 2145 & 25740 & 135135 & 270270 & 135135 &   & 7905853580625 \\
				14 & 1 & 91 & 3003 & 45045 & 315315 & 945945 & 945945 & 135135 & 213458046676875 \\
				15 & 1 & 105 & 4095 & 75075 & 675675 & 2837835 & 4729725 & 2027025 & 6190283353629375 \\
				\hline
			\end{tabular}
		\end{table}

	\section{The planar mod-$m$ diagram monoid $\card{\pmodmon{m}{k}}$}
		\begin{definition}
			For each $m \in \posints$ and $k_1, k_2 \in \posints$, let $T_{\planarmon{\textswab{A}^{m}_{k}}}(m, k, k_1, k_2)$ denote the number of ways to $\pmodmon{m}{k}$-feasibly connect $k_1$ upper vertices to $k_2$ lower vertices using only transversals.
		\end{definition}

	\section{Triapsis Monoid $|\triapmon{k}|$}
		Let $T_{\triapmon{}}(k_1, k_2)$ be the number of ways to $\triapmon{k}$-feasibly connect $k_1$ upper vertices to $k_2$ lower vertices using only transversals.
		
		\begin{figure}[!ht]
			\caption{The 8 ways to $\triapmon{k}$-feasibly connect 6 upper vertices to 3 lower vertices using only transversals.}
			\label{fig:TriapFeasTrans}
			\vspace{5pt}
			\centering
			\input{chap_cardinalities/tikz/TriapFeasTrans.tex}
		\end{figure}
    	
		\begin{proposition} The numbers $T_{\triapmon{}}(k_1, k_2)$ satisfy the recurrence:
			\begin{align*}
				T_{\triapmon{}}(0, 0) =&\ 1 \\
				T_{\triapmon{}}(k, 0) =&\ T_{\triapmon{}}(0, k) = 0 & \quad \text{ if } k > 0 \\
				T_{\triapmon{}}(k_1, k_2) =&\ 0 & \quad \text{ if } k_1 \not\equiv k_2 (\text{mod } 3) \\
				T_{\triapmon{}}(k_1, k_2) =&\ \sum_{\substack{(k_1', k_2') \leq (k_1, k_2)\\ k_1' \equiv k_2' (\text{mod } 3)}} T_{\triapmon{}}(k_1-k_1', k_2-k_2') & \quad \text{ if } k_1 \equiv k_2 (\text{mod } 3) 
			\end{align*}
			
			\begin{proof}
			 	Clearly we may not connect a positive number of vertices to zero vertices using transversals, nor may we $\triapmon{k}$-feasibly connect $k_1$ upper vertices with $k_2$ lower vertices using only transverals when $k_1 \not\equiv k_2 (\text{mod } 3)$. Suppose $k_1 \equiv k_2 (\text{mod } 3)$. If the transversal connected to the upper-right vertex connects the $k_1'$ upper right-most vertices and $k_2'$ lower right-most vertices, then there are $T_{\triapmon{}}(k_1-k_1', k_2-k_2')$ ways in which the remaining $k_1-k_1'$ upper vertices and $k_2-k_2'$ lower vertices may be $\triapmon{k}$-feasibly connected with transversals. Since there is one way for a single transversal to connect the $k_1$ upper vertices and $k_2$ lower vertices together it is convenient to have $T_{\triapmon{}}(0, 0) = 1$.
			\end{proof}
		\end{proposition}

		\begin{table}[!ht]
			\caption{Example values for $\noTrans{\triapmon{}}(k_1, k_2)$}
			\centering
			\tiny
			\begin{tabular}{| c | r r r r r r r r r r r r r |}
				\hline
				\diagbox{$k_1$}{$k_2$} & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
				\hline
				0  & 1 &   &   &    &    &     &     &     &     &      &      &      &      \\
				1  &   & 1 &   &    & 1  &     &     & 1   &     &      & 1    &      &      \\
				2  &   &   & 2 &    &    & 3   &     &     & 4   &      &      & 5    &      \\
				3  &   &   &   & 4  &    &     & 8   &     &     & 13   &      &      & 19   \\
				4  &   & 1 &   &    & 8  &     &     & 20  &     &      & 38   &      &      \\
				5  &   &   & 3 &    &    & 18  &     &     & 50  &      &      & 106  &      \\
				6  &   &   &   & 8  &    &     & 42  &     &     & 125  &      &      & 288  \\
				7  &   & 1 &   &    & 20 &     &     & 100 &     &      & 313  &      &      \\
				8  &   &   & 4 &    &    & 50  &     &     & 242 &      &      & 786  &      \\
				9  &   &   &   & 13 &    &     & 125 &     &     & 592  &      &      & 1979 \\
				10 &   & 1 &   &    & 38 &     &     & 313 &     &      & 1460 &      &      \\
				11 &   &   & 5 &    &    & 106 &     &     & 786 &      &      & 3624 &      \\
				12 &   &   &   & 19 &    &     & 288 &     &     & 1979 &      &      & 9042 \\
				\hline
			\end{tabular}
		\end{table}
    
        Let $\noNonTrans{\ppttnmon{}}(k, t_1, ..., t_m)$ be the number of ways to $\ppttnmon{k}$-feasibly place $t_1$ triapses, ..., and $t_m$ $3m$-apses along $k$ vertices.

        \begin{proposition} The numbers $\noNonTrans{\ppttnmon{}}(k, t_1, ..., t_m)$ satisfy the recurrence:
            \label{prop:noNonTransRecurrencesPlanarPttn}
            \begin{align*}
                \noNonTrans{\ppttnmon{}}(k, 0, ..., 0) =&\ 1 \\
                \noNonTrans{\ppttnmon{}}(k, t_1, ..., t_m) =&\ \noNonTrans{\ppttnmon{}}(k-1, t_1, ..., t_m) \\
                                                                                &+ \sum_{i:t_i > 0}\noNonTrans{\ppttnmon{}}(k-1, t_1, ..., t_i-1, ..., t_m)
            \end{align*}

            \begin{proof}
                There is only one way to place no apses, hence $\noNonTrans{\ppttnmon{}}(k, 0, ..., 0) = 1$. Suppose there is at least one apsis to be placed. If no apses connect to the right-most vertex then there are $\noNonTrans{\ppttnmon{}}(k-1, t_1, ..., t_m)$ ways to $\ppttnmon{k}$-feasibly place the $t_1$ triapses, ..., and $t_m$ $3m$-apses along the $k-1$ left-most vertices. If a $3i$-apsis $a$ is connected to the right-most vertex, then there are $\noNonTrans{\ppttnmon{}}(k-1, t_1, ..., t_i-1, ..., t_m)$ ways to $\ppttnmon{k}$-feasibly place the remaining $t_1$ triapses, ..., $t_i-1$ $3i$-apses, ..., and $t_m$ $3m$-apses along the $k-1$ left-most vertices, after which the $3i$-apsis $a$ is placed along the $3i$ right-most vertices. 
            \end{proof}
        \end{proposition}
        
        \begin{table}[!ht]
            \caption{Example values for $\noNonTrans{\ppttnmon{}}(k, \vec{t})$ where $\vec{t} = (t_1, t_2, t_3, t_4)$.}
            \centering \tiny
            \begin{tabular}{| c | r r r r r r r r r r r r |}
                \hline
                \diagbox{$k$}{$\vec{t}$} & \rotatebox{90}{(0,0,0,0) } & \rotatebox{90}{(1,0,0,0)} & \rotatebox{90}{(2,0,0,0)} & \rotatebox{90}{(3,0,0,0)} & \rotatebox{90}{(4,0,0,0)} & \rotatebox{90}{(0,1,0,0)} & \rotatebox{90}{(1,1,0,0)} & \rotatebox{90}{(2,1,0,0)} & \rotatebox{90}{(0,2,0,0)} & \rotatebox{90}{(0,0,1,0)} & \rotatebox{90}{(1,0,1,0)} & \rotatebox{90}{(0,0,0,1)} \\
                \hline
                0  & 1 &    &    &     &     &    &     &     &    &   &    &   \\
                1  & 1 &    &    &     &     &    &     &     &    &   &    &    \\
                2  & 1 &    &    &     &     &    &     &     &    &   &    &   \\
                3  & 1 & 1  &    &     &     &    &     &     &    &   &    &   \\
                4  & 1 & 2  &    &     &     &    &     &     &    &   &    &   \\
                5  & 1 & 3  &    &     &     &    &     &     &    &   &    &   \\
                6  & 1 & 4  & 3  &     &     & 1  &     &     &    &   &    &   \\
                7  & 1 & 5  & 7  &     &     & 2  &     &     &    &   &    &   \\
                8  & 1 & 6  & 12 &     &     & 3  &     &     &    &   &    &   \\
                9  & 1 & 7  & 18 & 12  &     & 4  & 9   &     &    & 1 &    &   \\
                10 & 1 & 8  & 25 & 30  &     & 5  & 20  &     &    & 2 &    &   \\
                11 & 1 & 9  & 33 & 55  &     & 6  & 33  &     &    & 3 &    &   \\
                12 & 1 & 10 & 42 & 88  & 55  & 7  & 48  & 66  & 6  & 4 & 12 & 1 \\
                13 & 1 & 11 & 52 & 130 & 143 & 8  & 65  & 156 & 13 & 5 & 26 & 2 \\
                14 & 1 & 12 & 63 & 182 & 273 & 9  & 84  & 273 & 21 & 6 & 42 & 3 \\
                15 & 1 & 13 & 75 & 245 & 455 & 10 & 105 & 420 & 30 & 7 & 60 & 4 \\
                \hline
            \end{tabular}
        \end{table}
        
        Let $\noNonTrans{\triapmon{}}(k, t_1, ..., t_m)$ be the number of ways to $\triapmon{k}$-feasibly place $t_1$ triapses, ..., and $t_m$ $3m$-apses along $k$ vertices. Ie. so that $t_1 > 0$ and at least one of the triapses connects consecutive vertices. 

        Note $(\noNonTrans{\ppttnmon{}} - \noNonTrans{\triapmon{}})(k, t_1, ..., t_m)$ is the number of ways to $\ppttnmon{k}$-feasibly place $t_1$ triapses, ..., and $t_m$ $3m$-apses along $k$ vertices such that no triapses connect consecutive vertices.

        \begin{proposition} The numbers $\noNonTrans{\triapmon{}}(k, t_1, ..., t_m)$ satisfy the recurrence:
            \begin{align*}
                \noNonTrans{\triapmon{}}(k, 0, ..., 0) =&\ 1 \\
                \noNonTrans{\triapmon{}}(k, 0, t_2, ..., t_m) =&\ 0 \\
                \noNonTrans{\triapmon{}}(k, t_1, ..., t_m) =&\ \noNonTrans{\triapmon{}}(k-1, t_1, ..., t_m) + (\noNonTrans{\ppttnmon{}} - \noNonTrans{\triapmon{}})(k-3, t_1-1, ..., t_m) \\
                                                                                    &+ \sum_{i:t_i > 0}\noNonTrans{\triapmon{}}(k-1, t_1, ..., t_i-1, ..., t_m)
            \end{align*}
				
            \begin{proof}
            	There is only one way to place no apses, hence $\noNonTrans{\triapmon{}}(k, 0, ..., 0) = 1$. Suppose there is at least one apsis to be placed. If none of the apses are triapses then we cannot $\triapmon{k}$-feasibly place the rest of the apses. If no apses connect to the right-most vertex then there are $\noNonTrans{\triapmon{}}(k-1, t_1, ..., t_m)$ ways to $\triapmon{k}$-feasibly place the $t_1$ triapses, ..., and $t_m$ $3m$-apses along the $k-1$ left-most vertices. If a $3i$-apsis $a$ is connected to the right-most vertex, then there are $\noNonTrans{\triapmon{}}(k-1, t_1, ..., t_i-1, ..., t_m)$ ways to $\triapmon{k}$-feasibly place the remaining $t_1$ triapses, ..., $t_i-1$ $3i$-apses, ..., and $t_m$ $3m$-apses along the $k-1$ left-most vertices, after which the $3i$-apsis $a$ is placed along the $3i$ right-most vertices. Note however if $a$ is a triapsis and connects the three right-most vertices then we have only counted the cases where at least two triapses connect consecutive vertices. We must also add the $(\noNonTrans{\ppttnmon{}} - \noNonTrans{\triapmon{}})(k-3, t_1-1, ..., t_m)$ ways to $\ppttnmon{k}$-feasibly place the remaining $t_1-1$ triapses, ..., and $t_m$ $3m$-apses along the $k-3$ left-most vertices such that no triapses connect consecutive vertices.
            \end{proof}
        \end{proposition}

        \begin{table}[!ht]
            \caption{Example values for $\noNonTrans{\triapmon{}}(k, \vec{t})$ where $\vec{t} = (t_1, t_2, t_3, t_4)$.}
            \centering \tiny
            \begin{tabular}{| c | r r r r r r r r r r r r |}
                \hline
                \diagbox{$k$}{$\vec{t}$} & \rotatebox{90}{(0,0,0,0) } & \rotatebox{90}{(1,0,0,0)} & \rotatebox{90}{(2,0,0,0)} & \rotatebox{90}{(3,0,0,0)} & \rotatebox{90}{(4,0,0,0)} & \rotatebox{90}{(0,1,0,0)} & \rotatebox{90}{(1,1,0,0)} & \rotatebox{90}{(2,1,0,0)} & \rotatebox{90}{(0,2,0,0)} & \rotatebox{90}{(0,0,1,0)} & \rotatebox{90}{(1,0,1,0)} & \rotatebox{90}{(0,0,0,1)} \\
                \hline
                0  & 1 &    &    &     &     &   &    &     &   &   &    &   \\
                1  & 1 &    &    &     &     &   &    &     &   &   &    &   \\
                2  & 1 &    &    &     &     &   &    &     &   &   &    &   \\
                3  & 1 & 1  &    &     &     &   &    &     &   &   &    &   \\
                4  & 1 & 2  &    &     &     &   &    &     &   &   &    &   \\
                5  & 1 & 3  &    &     &     &   &    &     &   &   &    &   \\
                6  & 1 & 4  & 3  &     &     & 0 &    &     &   &   &    &   \\
                7  & 1 & 5  & 7  &     &     & 0 &    &     &   &   &    &   \\
                8  & 1 & 6  & 12 &     &     & 0 &    &     &   &   &    &   \\
                9  & 1 & 7  & 18 & 12  &     & 0 & 7  &     &   & 0 &    &   \\
                10 & 1 & 8  & 25 & 30  &     & 0 & 16 &     &   & 0 &    &   \\
                11 & 1 & 9  & 33 & 55  &     & 0 & 27 &     &   & 0 &    &   \\
                12 & 1 & 10 & 42 & 88  & 55  & 0 & 40 & 62  & 0 & 0 & 10 & 0 \\
                13 & 1 & 11 & 52 & 130 & 143 & 0 & 55 & 148 & 0 & 0 & 22 & 0 \\
                14 & 1 & 12 & 63 & 182 & 273 & 0 & 72 & 261 & 0 & 0 & 36 & 0 \\
                15 & 1 & 13 & 75 & 245 & 455 & 0 & 91 & 404 & 0 & 0 & 52 & 0 \\
                \hline
            \end{tabular}
        \end{table}

        Let $\noNonTrans{\triapmon{}}(k, t) = \Sigma_{t_1 + ... + t_m = t: t_1 > 1} \noNonTrans{\triapmon{}}(k, t_1, ..., t_m)$ be the number of ways to $\triapmon{k}$-feasibly have $t$ of $k$ vertices connected to non-transversals. 

        \begin{theorem}
            The cardinality of $\triapmon{k}$ is given by:
            \[ |\triapmon{k}| = 1 + \sum_{u=1}^{\floor{k/3}}\sum_{l=1}^{\floor{k/3}} \noNonTrans{\triapmon{}}(k, 3u)\noNonTrans{\triapmon{}}{\triapmon{}}(k, 3l)T_{\triapmon{}}(k-3u, k-3l) \]

            \begin{proof}
				The identity is the only diagram $\alpha \in \triapmon{k}$ with $\rank{\alpha} = k$. Suppose the number of upper and lower vertices connected to non-transverals are $3u$ and $3l$ respectively, where $u, l \in \set{1, ..., \floor{\frac{k}{3}}}$. For each of the $\noNonTrans{\triapmon{}}(k, 3u)$ ways to $\triapmon{k}$-feasibly have $3u$ of $k$ upper vertices connected to non-transversals and $\noNonTrans{\triapmon{}}(k, 3l)$ ways to $\triapmon{k}$-feasibly have $3l$ of $k$ lower vertices connected to non-transversals, there are $T_{\triapmon{}}(k-3u, k-3l)$ ways to $\triapmon{k}$-feasibly connect the remaining $k-3u$ upper vertices to the remaining $k-3l$ lower vertices using only transversals.
            \end{proof}
        \end{theorem}
 
        \begin{table}[!ht]
            \caption{Example values for $\noNonTrans{\triapmon{}}(k, t)$ and $|\triapmon{k}|$.}
            \centering
            \tiny
            \begin{tabular}{|c|rrrr|c|}
                \hline
                \diagbox{k}{t} & 3 & 6 & 9 & 12 & $|\triapmon{k}|$ \\
                \hline
                3 & 1 &   &   &   & 1 \\
                4 & 2 &   &   &   & 4 \\
                5 & 3 &   &   &   & 18 \\
                6 & 4 & 3 &   &   & 73 \\
                7 & 5 & 7 &   &   & 319 \\
                8 & 6 & 12 &   &   & 1368 \\
                9 & 7 & 18 & 19 &   & 5731 \\
                10 & 8 & 25 & 46 &   & 24552 \\
                11 & 9 & 33 & 82 &   & 104492 \\
                12 & 10 & 42 & 128 & 127 & 439249 \\
                13 & 11 & 52 & 185 & 313 & 1871609 \\
                14 & 12 & 63 & 254 & 570 & 7952610 \\
                15 & 13 & 75 & 336 & 911 & 33550196 \\
                \hline
            \end{tabular}
        \end{table}
\begin{comment}
    \section{Fauser Monoid $|\fausermon{k}|$}
    	Let $T_{\fausermon{}}(k_1, k_2)$ be the number of ways to $\fausermon{k}$-feasibly connect $k_1$ upper vertices to $k_2$ lower vertices using only transversals.
    	
		\begin{proposition} The numbers $T_{\fausermon{}}(k_1, k_2)$ satisfy the recurrence:
			\begin{align*}
				T_{\fausermon{}}(0, 0) =&\ 1 \\
				T_{\fausermon{}}(k, 0) =&\ T_{\fausermon{}}(0, k) = 0 \text{ if } k > 0 \\
				T_{\fausermon{}}(k_1, k_2) =&\ 0 \text{ if } k_1 \not\equiv k_2 (\text{mod } 3) \\
				T_{\fausermon{}}(k_1, k_2) =&\ \sum_{\substack{(k_1', k_2') \leq (k_1, k_2)\\ k_1' \equiv k_2' (\text{mod } 3)}} \binom{k_1-1}{k_1'-1}\binom{k_2}{k_2'}T_{\fausermon{}}(k_1-k_1', k_2-k_2')
			\end{align*}
			
			\begin{proof}
				Clearly we may not connect a positive number of vertices to zero vertices using transversals, nor can we $\fausermon{k}$-feasibly connect $k_1$ upper vertices with $k_2$ lower vertices using only transverals when $k_1 \not\equiv k_2 (\text{mod } 3)$. Suppose $k_1 \equiv k_2 (\text{mod } 3)$. Suppose the transversal connected to the upper-right vertex connects $k_1'$ upper vertices and $k_2'$ lower vertices, for each of the $\binom{k_1-1}{k_1'-1}\binom{k_2}{k_2'}$ ways in which this may happen, there are $T_{\fausermon{}}(k_1-k_1', k_2-k_2')$ ways in which the remaining $k_1-k_1'$ upper vertices and $k_2-k_2'$ lower vertices may be $\fausermon{k}$-feasibly connected with transversals. Since there is one way for a single transversal to connect the $k_1$ upper vertices and $k_2$ lower vertices together it is convenient to have $T_{\fausermon{}}(0, 0) = 1$.
			\end{proof}
		\end{proposition}
		
		\begin{table}[!ht]
			\caption{Example values for $\noTrans{\fausermon{}}(k_1, k_2)$}
			\centering
			\tiny
			\begin{tabular}{|c|rrrrrrrrrr|}
				\hline
				\diagbox{$k_1$}{$k_2$} & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\
				\hline
				0 & 1 &   &   &   &   &   &   &   &   &   \\
				1 &   & 1 &   &   & 1 &   &   & 1 &   &   \\
				2 &   &   & 3 &   &   & 11 &   &   & 87 &   \\
				3 &   &   &   & 16 &   &   & 154 &   &   & 2620 \\
				4 &   & 1 &   &   & 131 &   &   & 2647 &   &   \\
				5 &   &   & 11 &   &   & 1521 &   &   & 55731 &   \\
				6 &   &   &   & 154 &   &   & 23562 &   &   & 1419082 \\
				7 &   & 1 &   &   & 2647 &   &   & 469659 &   &   \\
				8 &   &   & 87 &   &   & 55731 &   &   & 11676227 &   \\
				9 &   &   &   & 2620 &   &   & 1419082 &   &   & 353355424 \\
				\hline
			\end{tabular}
		\end{table}
    
        Let $N_{\pttnmon{}}(k, t_1, ..., t_m)$ be the number of ways to $\pttnmon{k}$-feasibly place $t_1$ triapses, ..., and $t_m$ $3m$-apses along $k$ vertices.

        \begin{proposition} The numbers $N_{\pttnmon{}}(k, t_1, ..., t_m)$ satisfy the recurrence:
            \begin{align*}
                N_{\pttnmon{}}(k, 0, ..., 0) =&\ 1 \\
                N_{\pttnmon{}}(k, t_1, ..., t_m) =&\ N_{\pttnmon{}}(k-1, t_1, ..., t_m) \\
                                               &+ \sum_{i:t_i > 0}\binom{k-1}{3i-1}N_{\pttnmon{}}(k-3i, t_1, ..., t_i-1, ..., t_m)
            \end{align*}

            \begin{proof}
                There is only one way to place no apses, hence $\noNonTrans{\pttnmon{}}(k, 0, ..., 0) = 1$. Suppose there is at least one apsis to be placed. If no apses connect to the right-most vertex then there are $\noNonTrans{\pttnmon{}}(k-1, t_1, ..., t_m)$ ways to $\pttnmon{k}$-feasibly place the $t_1$ triapses, ..., and $t_m$ $3m$-apses along the $k-1$ left-most vertices. For each of the $\binom{k-1}{3i-1}$ ways a $3i$-apsis may connect to the right-most vertex, there are $N_{\pttnmon{}}(k-3i, t_1, ..., t_i-1, ..., t_m)$ ways to $\pttnmon{k}$-feasibly place the remaining $t_1$ triapses, ..., $t_i-1$ $3i$-apses, ..., and $t_m$ $3m$-apses along the remaining $k-3i$ vertices.
            \end{proof}
        \end{proposition}
        
        \begin{proposition} The numbers $N_{\fausermon{}}(k, t_1, ..., t_m)$ satisfy the recurrence:
            \begin{align*}
                N_{\fausermon{}}(k, 0, ..., 0) =&\ 1 \\
                N_{\fausermon{}}(k, 0, t_2, ..., t_m) =&\ 0 \\
                N_{\fausermon{}}(k, t_1, ..., t_m) =&\ N_{\pttnmon{}}(k, t_1, ..., t_m) \\
            \end{align*}

            \begin{proof}	
            \end{proof}
        \end{proposition}
        
        \begin{table}[!ht]
            \caption{Example values for $\noNonTrans{\pttnmon{}}(k, \vec{t})$ where $\vec{t} = (t_1, t_2, t_3)$.}
            \centering \tiny
            \begin{tabular}{|c|rrrrrrr|}
                \hline
                \diagbox{$k$}{$\vec{t}$} & \rotatebox{90}{(0,0,0) } & \rotatebox{90}{(1,0,0)} & \rotatebox{90}{(2,0,0)} & \rotatebox{90}{(3,0,0)} & \rotatebox{90}{(0,1,0)} & \rotatebox{90}{(1,1,0)} & \rotatebox{90}{(0,0,1)}  \\
                \hline
                0 & 1 &   &   &   &   &   &   \\
                1 & 1 &   &   &   &   &   &   \\
                2 & 1 &   &   &   &   &   &   \\
                3 & 1 & 1 &   &   &   &   &   \\
                4 & 1 & 4 &   &   &   &   &   \\
                5 & 1 & 10 &   &   &   &   &   \\
                6 & 1 & 20 & 10 &   & 1 &   &   \\
                7 & 1 & 35 & 70 &   & 7 &   &   \\
                8 & 1 & 56 & 280 &   & 28 &   &   \\
                9 & 1 & 84 & 840 & 280 & 84 & 84 & 1 \\
                10 & 1 & 120 & 2100 & 2800 & 210 & 840 & 10 \\
                11 & 1 & 165 & 4620 & 15400 & 462 & 4620 & 55 \\
                \hline
            \end{tabular}
        \end{table}

        Let $N_{\fausermon{}}(k, t) = \Sigma_{t_1 + ... + t_m = t: t_1 > 1} N_{\pttnmon{}}(k, t_1, ..., t_m)$ be the number of ways to $\fausermon{k}$-feasibly have $t$ of $k$ vertices connected to non-transversals. 
        
        \begin{table}[!ht]
            \caption{Example values for $\noNonTrans{\fausermon{}}(k, t)$ and $|\fausermon{k}|$.}
            \centering
            \tiny
            \begin{tabular}{|c|rrr|c|}
                \hline
                \diagbox{k}{t} & 3 & 6 & 9 & $|\fausermon{k}|$ \\
                \hline
                0 &   &   &   & 0 \\
                1 &   &   &   & 0 \\
                2 &   &   &   & 0 \\
                3 & 1 &   &   & 7 \\
                4 & 4 &   &   & 40 \\
                5 & 10 &   &   & 420 \\
                6 & 20 & 10 &   & 7220 \\
                7 & 35 & 70 &   & 175315 \\
                8 & 56 & 280 &   & 5390336 \\
                9 & 84 & 840 & 364 & 199770928 \\
                10 & 120 & 2100 & 3640 & 8707927600 \\
                11 & 165 & 4620 & 20020 & 439169520075 \\
                \hline
            \end{tabular}
        \end{table}

        \begin{theorem}
            The cardinality of $\fausermon{k}$ is given by:
            \[ |\fausermon{k}| = k! + \sum_{u=1}^{\floor{k/3}}\sum_{l=1}^{\floor{k/3}} N_{\fausermon{}}(k, 3u)N_{\fausermon{}}(k, 3l)T_{\fausermon{}}(k-3u, k-3l) \]
            \begin{proof}
            	There are $k!$ diagrams $\alpha \in \fausermon{k}$ with $\rank{\alpha} = k$, namely the symmetric group $\symgrp{k}$. Suppose the number of upper and lower vertices connected to non-transverals are $3u$ and $3l$ respectively, where $u, l \in \set{1, ..., \floor{\frac{k}{3}}}$. For each of the $\noNonTrans{\fausermon{}}(k, 3u)$ ways to $\fausermon{k}$-feasibly have $3u$ of $k$ upper vertices connected to non-transversals and $\noNonTrans{\fausermon{}}(k, 3l)$ ways to $\fausermon{k}$-feasibly have $3l$ of $k$ lower vertices connected to non-transversals, there are $T_{\fausermon{}}(k-3u, k-3l)$ ways to $\fausermon{k}$-feasibly connect the remaining $k-3u$ upper vertices to the remaining $k-3l$ lower vertices using only transversals.
            \end{proof}
        \end{theorem}
\end{comment}

==> chap_characterisations/tikz/fig-template.tex <==
\begin{tikzpicture} [scale = 0.6]
	\begin{scope} [shift={(0,2)}]
		% % % % % % % % %
		%%g1 

	\end{scope}
	
	\begin{scope} [shift={(0,0)}]
		% % % % % % % % %
		% %g3
	
	\end{scope}
	
\end{tikzpicture}


==> chap_introduction/tikz/fig_introexample.tex <==
\begin{tikzpicture}[scale = 0.6]
	\begin{scope}[shift={(0,5.5)}]
		\draw(-0.5, 1) node {$\alpha$};
		%block #1
		%vertices and labels
		\fill(1,2)circle(.125);
		\fill(2,2)circle(.125);

		%lines
		\draw(1,1.875) .. controls (1,1.46154) and (2,1.46154) .. (2,1.875);

		%block #2
		%vertices and labels
		\fill(3,2)circle(.125);
		\fill(4,0)circle(.125);

		%lines
		\draw(3,2)--(4,0);

		%block #3
		%vertices and labels
		\fill(4,2)circle(.125);
		\fill(5,0)circle(.125);

		%lines
		\draw(4,2)--(5,0);

		%block #4
		%vertices and labels
		\fill(5,2)circle(.125);
		\fill(6,0)circle(.125);

		%lines
		\draw(5,2)--(6,0);

		%block #5
		%vertices and labels
		\fill(6,2)circle(.125);

		%lines

		%block #6
		%vertices and labels
		\fill(7,2)circle(.125);
		\fill(7,0)circle(.125);

		%lines
		\draw(7,2)--(7,0);

		%block #7
		%vertices and labels
		\fill(8,2)circle(.125);
		\fill(13,0)circle(.125);

		%lines
		\draw(8,2)--(9,1);
		\draw(9,1)--(12,1);
		\draw(12,1)--(13,0);

		%block #8
		%vertices and labels
		\fill(9,2)circle(.125);
		\fill(10,2)circle(.125);
		\fill(11,2)circle(.125);
		\fill(12,2)circle(.125);
		\fill(13,2)circle(.125);

		%lines
		\draw(9,1.875) .. controls (9,1.46154) and (10,1.46154) .. (10,1.875);
		\draw(10,1.875) .. controls (10,1.46154) and (11,1.46154) .. (11,1.875);
		\draw(11,1.875) .. controls (11,1.46154) and (12,1.46154) .. (12,1.875);
		\draw(12,1.875) .. controls (12,1.46154) and (13,1.46154) .. (13,1.875);

		%block #9
		%vertices and labels
		\fill(1,0)circle(.125);
		\fill(2,0)circle(.125);
		\fill(3,0)circle(.125);

		%lines
		\draw(1,0.125) .. controls (1,0.538462) and (2,0.538462) .. (2,0.125);
		\draw(2,0.125) .. controls (2,0.538462) and (3,0.538462) .. (3,0.125);

		%block #10
		%vertices and labels
		\fill(8,0)circle(.125);
		\fill(12,0)circle(.125);

		%lines
		\draw(8,0.125) .. controls (8,0.9) and (12,0.9) .. (12,0.125);

		%block #11
		%vertices and labels
		\fill(9,0)circle(.125);
		\fill(10,0)circle(.125);

		%lines
		\draw(9,0.125) .. controls (9,0.538462) and (10,0.538462) .. (10,0.125);

		%block #12
		%vertices and labels
		\fill(11,0)circle(.125);

		%lines
	\end{scope}
	
	\begin{scope}[shift={(0,3.5)}]
		\draw(-0.5, 1) node {$\beta$};
		%block #1
		%vertices and labels
		\fill(1,2)circle(.125);
		\fill(2,2)circle(.125);
		\fill(3,2)circle(.125);

		%lines
		\draw(1,1.875) .. controls (1,1.46154) and (2,1.46154) .. (2,1.875);
		\draw(2,1.875) .. controls (2,1.46154) and (3,1.46154) .. (3,1.875);

		%block #2
		%vertices and labels
		\fill(4,2)circle(.125);
		\fill(7,2)circle(.125);
		\fill(3,0)circle(.125);

		%lines
		\draw(4,1.875) .. controls (4,1.1) and (7,1.1) .. (7,1.875);
		\draw(4,2)--(3,0);

		%block #3
		%vertices and labels
		\fill(5,2)circle(.125);
		\fill(6,2)circle(.125);

		%lines
		\draw(5,1.875) .. controls (5,1.46154) and (6,1.46154) .. (6,1.875);

		%block #4
		%vertices and labels
		\fill(8,2)circle(.125);
		\fill(4,0)circle(.125);
		\fill(7,0)circle(.125);
		\fill(8,0)circle(.125);

		%lines
		\draw(4,0.125) .. controls (4,0.9) and (7,0.9) .. (7,0.125);
		\draw(7,0.125) .. controls (7,0.538462) and (8,0.538462) .. (8,0.125);
		\draw(8,2)--(8,0);

		%block #5
		%vertices and labels
		\fill(9,2)circle(.125);

		%lines

		%block #6
		%vertices and labels
		\fill(10,2)circle(.125);
		\fill(11,2)circle(.125);

		%lines
		\draw(10,1.875) .. controls (10,1.46154) and (11,1.46154) .. (11,1.875);

		%block #7
		%vertices and labels
		\fill(12,2)circle(.125);
		\fill(13,2)circle(.125);
		\fill(11,0)circle(.125);

		%lines
		\draw(12,1.875) .. controls (12,1.46154) and (13,1.46154) .. (13,1.875);
		\draw(12,2)--(11,0);

		%block #8
		%vertices and labels
		\fill(1,0)circle(.125);
		\fill(2,0)circle(.125);

		%lines
		\draw(1,0.125) .. controls (1,0.538462) and (2,0.538462) .. (2,0.125);

		%block #9
		%vertices and labels
		\fill(5,0)circle(.125);
		\fill(6,0)circle(.125);

		%lines
		\draw(5,0.125) .. controls (5,0.538462) and (6,0.538462) .. (6,0.125);

		%block #10
		%vertices and labels
		\fill(9,0)circle(.125);
		\fill(10,0)circle(.125);

		%lines
		\draw(9,0.125) .. controls (9,0.538462) and (10,0.538462) .. (10,0.125);

		%block #11
		%vertices and labels
		\fill(12,0)circle(.125);
		\fill(13,0)circle(.125);

		%lines
		\draw(12,0.125) .. controls (12,0.538462) and (13,0.538462) .. (13,0.125);
	\end{scope}
	
	\begin{scope}[shift={(0,0)}]
		\draw(-0.5, 1) node {$\alpha\beta$};
		\draw(7, 2.75) node {$\verteq$};
		%block #1
		%vertices and labels
		\fill(1,2)circle(.125);
		\fill(2,2)circle(.125);

		%lines
		\draw(1,1.875) .. controls (1,1.46154) and (2,1.46154) .. (2,1.875);

		%block #2
		%vertices and labels
		\fill(3,2)circle(.125);
		\fill(7,2)circle(.125);
		\fill(3,0)circle(.125);

		%lines
		\draw(3,1.875) .. controls (3,1.1) and (7,1.1) .. (7,1.875);
		\draw(3,2)--(3,0);

		%block #3
		%vertices and labels
		\fill(4,2)circle(.125);
		\fill(5,2)circle(.125);

		%lines
		\draw(4,1.875) .. controls (4,1.46154) and (5,1.46154) .. (5,1.875);

		%block #4
		%vertices and labels
		\fill(6,2)circle(.125);

		%lines

		%block #5
		%vertices and labels
		\fill(8,2)circle(.125);
		\fill(4,0)circle(.125);
		\fill(7,0)circle(.125);
		\fill(8,0)circle(.125);
		\fill(11,0)circle(.125);

		%lines
		\draw(4,0.125) .. controls (4,0.9) and (7,0.9) .. (7,0.125);
		\draw(7,0.125) .. controls (7,0.538462) and (8,0.538462) .. (8,0.125);
		\draw(8,0.125) .. controls (8,0.9) and (11,0.9) .. (11,0.125);
		\draw(8,2)--(8,0);

		%block #6
		%vertices and labels
		\fill(9,2)circle(.125);
		\fill(10,2)circle(.125);
		\fill(11,2)circle(.125);
		\fill(12,2)circle(.125);
		\fill(13,2)circle(.125);

		%lines
		\draw(9,1.875) .. controls (9,1.46154) and (10,1.46154) .. (10,1.875);
		\draw(10,1.875) .. controls (10,1.46154) and (11,1.46154) .. (11,1.875);
		\draw(11,1.875) .. controls (11,1.46154) and (12,1.46154) .. (12,1.875);
		\draw(12,1.875) .. controls (12,1.46154) and (13,1.46154) .. (13,1.875);

		%block #7
		%vertices and labels
		\fill(1,0)circle(.125);
		\fill(2,0)circle(.125);

		%lines
		\draw(1,0.125) .. controls (1,0.538462) and (2,0.538462) .. (2,0.125);

		%block #8
		%vertices and labels
		\fill(5,0)circle(.125);
		\fill(6,0)circle(.125);

		%lines
		\draw(5,0.125) .. controls (5,0.538462) and (6,0.538462) .. (6,0.125);

		%block #9
		%vertices and labels
		\fill(9,0)circle(.125);
		\fill(10,0)circle(.125);

		%lines
		\draw(9,0.125) .. controls (9,0.538462) and (10,0.538462) .. (10,0.125);

		%block #10
		%vertices and labels
		\fill(12,0)circle(.125);
		\fill(13,0)circle(.125);

		%lines
		\draw(12,0.125) .. controls (12,0.538462) and (13,0.538462) .. (13,0.125);
	\end{scope}
\end{tikzpicture}


==> chap_introduction/tikz/fig_matrixgrpsanddiagalgebras.tex <==
\begin{tikzpicture}[scale = 0.8]
\draw [fill=blue!15,rounded corners] (-1.5,-1.5)--(1.5,-1.5)--(1.5,4.75)--(-1.5,4.75)--cycle;
\draw (0,-1) node {{\footnotesize Matrix groups}};
\draw [fill=blue!15,rounded corners] (-1.75+5,-1.5)--(1.75+5,-1.5)--(1.75+5,4.75)--(-1.75+5,4.75)--cycle;
\draw (0+5,-1) node {{\footnotesize Diagram algebras}};
\path
(0,6) node(c) [rectangle,rounded corners=3pt,draw,fill=blue!30] {${\text{General} \atop \text{linear group}}$}
(0,4) node(b) [rectangle,rounded corners=3pt,draw,fill=blue!30] {${\text{Orthogonal} \atop \text{group}}$}
(0,2) node(b) [rectangle,rounded corners=3pt,draw,fill=blue!30] {${\text{Orthogonal} \atop \text{group}}$}
(0,0) node(a) [rectangle,rounded corners=3pt,draw,fill=blue!30] {${\text{Symmetric} \atop \text{group}}$}
(5,6) node(f) [rectangle,rounded corners=3pt,draw,fill=blue!30] {${\text{Symmetric} \atop \text{group algebra}}$}
(5,4) node(e) [rectangle,rounded corners=3pt,draw,fill=blue!30] {${\text{Brauer} \atop \text{algebra}}$}
(5,2) node(e) [rectangle,rounded corners=3pt,draw,fill=blue!30] {${\text{Mod-$2$} \atop \text{algebra}}$}
(5,0) node(d) [rectangle,rounded corners=3pt,draw,fill=blue!30] {${\text{Partition} \atop \text{algebra}}$}
;
\draw[thick,{latex}-{latex}] (c) -- (f);
\draw[thick,{latex}-{latex}] (b) -- (e);
\draw[thick,{latex}-{latex}] (a) -- (d);
\draw[thick,-{latex}] (a) -- (b);
\draw[thick,-{latex}] (b) -- (c);
\draw[thick,-{latex}] (f) -- (e);
\draw[thick,-{latex}] (e) -- (d);
\end{tikzpicture}

